Improving Interpretability via Explicit Word Interaction Graph Layer

Recent NLP literature has seen growing interest in improving model interpretability. Along this direction, we propose a trainable neural network layer that learns a global interaction graph between words and then selects more informative words using the learned word interactions. Our layer, we call WIGRAPH, can plug into any neural network-based NLP text classifiers right after its word embedding layer. Across multiple SOTA NLP models and various NLP datasets, we demonstrate that adding the WIGRAPH layer substantially improves NLP models' interpretability and enhances models' prediction performance at the same time.

==> 036cooccur.tex <==
\subsection{Using co-occurrence matrix}
We define a co-occurrence matrix, a matrix of size $V\times V$ that counts the number of times each word $i$ co-occurs with another word $j$ in a sentence over the entire training dataset. Concretely, for each word $w_i$ in a sentence, and each word in the sentence, we $C[i,j]+=1$ if the two words occur together in the sentence. 
We further convert this into an initial probability using:
Say each training sample is represented by 
$v_i$ is a one-hot vector indicating the presence or absence of a word in a vocabulary in a training sample $i$. and $n_i = \sum_{j=1}^V v_{ij}$. 
We investigate two types of co occurrence statistics:



(1) \begin{equation}
    \mathbf{C} = \dfrac{Count(w_i, w_j) }{\sum_{i=1}^{|V|} \sum_{j=1}^{|V|}Count(w_i, w_j) }
\end{equation}
We use the co-occurrence as a prior instead of a Bernoulli parameter for the KL term between $\mathbf{A}$. 



==> 039methodMore.tex <==
\subsection{More Details about Method}
\label{sec:moremethod}



==> table_ablation_aopc_short.tex <==
\subsection{Additional Experimentation: Ablation Analysis for Interpretation Scores}
\begin{table}[h]
	\centering
\begin{minipage}[]{\hsize}
\centering
\scalebox{0.89}{
    \begin{tabular}{cccc}
		\toprule
		 Metric & Models & TREC & SST-2   \\
		\midrule
		\multirow{4}{*}{AOPC} & \base  & 67.63 & 42.25 \\	
		 & \vmask & 63.14 & 39.77 \\	
		 & \methodAR & 61.52 & 36.22 \\
		& \band \methodA & {\bf 68.74} & {\bf 44.33}\\
		\bottomrule
	\end{tabular}}
	\caption{Ablations analysis for TREC and SST-2 datasets on distilbert model regarding AOPC from LIME post-hoc explanation model for ablations \methodA and \methodAR. }
	\label{tab:ablations_aopc}
	\end{minipage} 

\end{table}
